On k-Mer-Based and Maximum Likelihood Estimation Algorithms for Trace Reconstruction

The goal of the trace reconstruction problem is to recover a string $x\in\{0,1\}^n$ given many independent {\em traces} of $x$, where a trace is a subsequence obtained from deleting bits of $x$ independently with some given probability $p\in [0,1).$ A recent result of Chase (STOC 2021) shows how $x$ can be determined (in exponential time) from $\exp(\widetilde{O}(n^{1/5}))$ traces. This is the state-of-the-art result on the sample complexity of trace reconstruction. In this paper we consider two kinds of algorithms for the trace reconstruction problem. Our first, and technically more involved, result shows that any $k$-mer-based algorithm for trace reconstruction must use $\exp(\Omega(n^{1/5}))$ traces, under the assumption that the estimator requires $poly(2^k, 1/\varepsilon)$ traces, thus establishing the optimality of this number of traces. The analysis of this result also shows that the analysis technique used by Chase (STOC 2021) is essentially tight, and hence new techniques are needed in order to improve the worst-case upper bound. Our second, simple, result considers the performance of the Maximum Likelihood Estimator (MLE), which specifically picks the source string that has the maximum likelihood to generate the samples (traces). We show that the MLE algorithm uses a nearly optimal number of traces, \ie, up to a factor of $n$ in the number of samples needed for an optimal algorithm, and show that this factor of $n$ loss may be necessary under general ``model estimation'' settings.

==> counting.tex <==
\subsection{Proof of \cref{lem:technical-main}: A Counting Argument}

We prove \cref{lem:technical-main} in this section. 

{
\color{red}

New stuff below.

\input{improved_Sbound}
}

The proof will focus on a set of strings defined as follows. Denote $\*s_0=0^{L^{1/3}-1}$. Let
\begin{align*}
    S \coloneqq \set{\*s_0 b_1\*s_0 b_2\dots\*s_0 b_{L^{2/3}-1}\*s_00 \colon b_1,\dots, b_{L^{2/3}-1} \in \set{0,1} }.
\end{align*}
It is easily verified that each string in $S$ has length exactly $L$, and that $\abs{S}=2^{L^{2/3}-1}$. The key property about $S$ is that for a string $\*x \in S$, any two 1s in $\*x$ are separated by at least $L^{1/3}-1$ 0s.

Below we characterize some properties of $k$-mer generating polynomials of strings in $S$.
\begin{lemma} \label{lem:set-properties}
Let $S$ be a set of strings defined as above. For $j=1,2,\dots,k$, denote by $\*e_j$ the string with a single ``1'' located at index $j-1$ (indices begin with 0). The following properties hold.
\begin{enumerate}
 \item For any $k$-mer $w \notin \set{0^k, \*e_1, \dots, \*e_k}$, $P_{w,\*x}(z)$ is the zero polynomial.
 \item For any $\*x \in S$ and $1\le j<k$, $P_{\*e_j,\*x}(z) = (p+(1-p)z)\cdot P_{\*e_{j+1},\*x}(z)$.
 \item For any $\*x, \*y \in S$ and $\abs{z}\le 1$, $\abs{P_{0^k, \*x}(z)-P_{0^k, \*y}(z)} \le k\cdot\abs{P_{\*e_k,\*x}(z)-P_{\*e_k,\*y}(z)}$ .
\end{enumerate}
\end{lemma}
\begin{proof}
\textit{Item 1:} By the property of $S$, $\*x[j:j-k+1]$ contains at most one ``1'' for any string $\*x \in S$. Therefore, if $w$ contains at least two ``1''s, then for any $0\le \ell<L-k$,  
\begin{align*}
    K_{w,\*x}[\ell] = \sum_{j=0}^{L-k}\binom{j}{\ell}p^{\ell}(1-p)^{j-\ell}\idc{\*x[j:j-k+1]=w} = 0.
\end{align*}
This means all the coefficients of $P_{w,\*x}(z)$ is zero, and hence $P_{w,\*x}(z)$ is the zero polynomial.

\textit{Item 2:} Since any two consecutive ``1''s in $\*x \in S$ are separated by at least $k-1$ ``0''s, $\*x[i:i+k-1]=\*e_j$ if and only if $\*x[i-1:i+k-2]=\*e_{j+1}$. We thus have
\begin{align*}
    P_{\*e_j,\*x}(z) &= \sum_{i=0}^{L-k} \idc{\*x[i:i+k-1]=\*e_j}\cdot (p+(1-p)z)^i \\
    &= \sum_{i=1}^{L-k} \idc{\*x[i-1:i+k-2]=\*e_{j+1}}\cdot (p+(1-p)z)^i \\
    &= (p+(1-p)z)\cdot \sum_{i=0}^{L-k-1} \idc{\*x[i:i+k-1]=\*e_{j+1}}\cdot (p+(1-p)z)^i \\
    &= (p+(1-p)z)\cdot P_{\*e_{j+1},\*x}(z).
\end{align*}
We have used the fact that for $1\le j< k$, $\idc{\*x[0:k-1]=\*e_j}=\idc{\*x[L-k:L-1]=\*e_{j+1}}=0$.

\textit{Item 3:} We observe that $\*x[i:i+k-1] \in \set{0^k, \*e_1, \dots, \*e_k}$. That implies
\begin{align*}
    \sum_{w \in \set{0^k, \*e_1, \dots, \*e_k}}P_{w,\*x}(z) &= \sum_{w \in \set{0^k, \*e_1, \dots, \*e_k}}\sum_{i=0}^{L-k} \idc{\*x[i:i+k-1]=w}\cdot (p+(1-p)z)^i \\
    &= \sum_{i=0}^{L-k} \tp{\sum_{w \in \set{0^k, \*e_1, \dots, \*e_k}} \idc{\*x[i:i+k-1]=w}}(p+(1-p)z)^i \\
    &= \sum_{i=0}^{L-k}(p+(1-p)z)^i.
\end{align*}
Note the the right-hand-side is independent of $\*x$. Therefore
\begin{align*}
    \abs{P_{0^k,\*x}(z)-P_{0^k,\*y}(z)} &= \abs{\sum_{w \in \set{\*e_1, \dots, \*e_k}}P_{w,\*x}(z) - \sum_{w \in \set{\*e_1, \dots, \*e_k}}P_{w,\*y}(z)} \\
    &\le \sum_{j=1}^{k}\abs{P_{\*e_j,\*x}(z)-P_{\*e_j,\*y}(z)} \\
    &= \sum_{j=1}^{k}\abs{\tp{p+(1-p)z}^{k-j}\cdot\tp{P_{\*e_k,\*x}(z)-P_{\*e_k,\*y}(z)}} \\
    &\le k\cdot \abs{P_{\*e_k,\*x}(z)-P_{\*e_k,\*y}(z)}.
\end{align*}
The second last line is obtained by inductively applying Item 2.
\end{proof}



Below we give the proof of \cref{lem:technical-main}. We use the notations $\exp(x)\coloneqq e^x$, and $\exp_2(x)\coloneqq 2^x$.

\begin{proof}[Proof of \cref{lem:technical-main}]
Let $\*x \in S$ be a string of length $L$. In light of \cref{lem:set-properties}, we only need to consider a fixed $k$-mer $w=\*e_k$, where $k\le L^{1/3}$. Define
\begin{align*}
	g_{\*x}(z) \coloneqq \sum_{j=0}^{L-k}\idc{\*x[j\colon j+k-1]=\*e_k}\cdot z^j.
\end{align*}
Recall that $g_{\*x}(p+qz)=\sum_{j=0}^{L-1}K_{\*e_k,\*x}[j]\cdot z^j=P_{\*e_k,\*x}(z)$. Denote by $a_0(\*x), \dots, a_{L-k}(\*x)$ the Chebyshev coefficients of 
\begin{align*}
	f_{\*x}(z) \coloneqq g_{\*x}(1-4a+4a\cdot z),
\end{align*}
where $a\coloneqq L^{-2/3}$ (equivalently, the coordinates of $f_{\*x}$ in the Chebyshev basis). In other words, we can write
\begin{align*}
	f_{\*x}(z) = \sum_{j=0}^{L-k}a_j(\*x) \cdot T_j(z).
\end{align*}
We first argue that only the first few coefficients are significant. This can be done by applying \cref{thm:chebcoef-bound} to $f_{\*x}(z)$, say, with $\rho=2$. To that end, we first upper bound $\abs{f_{\*x}(z)}$ for $z \in E_{2}$. Denoting $z'=1-4a+4a\cdot z$, we have that $z' \in \tE_{a,2}$ when $z\in E_2$. By item (1) of \cref{prop:ellipse-bound}, we have $\abs{z'}\le 1+a$. It follows that
\begin{align*}
    \sup_{z \in E_2}\abs{f_{\*x}(z)} = \sup_{z' \in \tE_{a,2}}\abs{g_{\*x}(z')} \le L(1+a)^L \le L\exp(aL) = L\exp(L^{1/3}).
\end{align*}
Therefore, we can apply \cref{thm:chebcoef-bound} to $f_{\*x}(z)$ with $\rho=2$,$M=L\exp(L^{1/3})$ and get
\begin{align*}
	\forall j\ge 2L^{1/3},\quad \abs{a_{j}(\*x)} \le 2L\exp(L^{1/3})\cdot 2^{-j} \le 2L\exp(L^{1/3})\cdot 2^{-2L^{1/3}} \le 2^{-L^{1/3}/4}.
\end{align*}

To each string $\*x \in \set{0,1}^{L}$ we associate a vector
\begin{align*}
	\phi(\*x) \coloneqq \tp{a_j(\*x)\colon j=0,1,\dots,2L^{1/3}-1}.
\end{align*}
\cref{prop:trivial-chebcoef-bound} implies each entry of $\phi(\*x)$ belongs to the interval $[-2(L-k+1),2(L-k+1)]\subseteq [-2L,2L]$. We now partition $[-2L, 2L]$ into $m$ smaller intervals $I_1, \dots, I_m$, each of length $2^{-L^{1/3}/4}$, meaning that $m=4L\cdot 2^{L^{1/3}/4}$. The vector $\phi(\*x)$ must fall into one of the sub-cubes of the form
\begin{align*}
	\+I(r) \coloneqq \prod_{0\le j< 2L^{1/3}}I_{r(j)},
\end{align*}
where $r\colon [2L^{1/3}] \rightarrow [m]$ is a mapping that uniquely identifies the sub-cube. It follows that the total number of such sub-cubes is
\begin{align*}
	m^{2L^{1/3}} &= \tp{4L\cdot 2^{L^{1/3}/4}}^{2L^{1/3}} \\
	&= \exp_2\tp{\tp{\frac{L^{1/3}}{4} + \log_2{L} + 2}\cdot 2L^{1/3}} \\
	&\le \exp_2\tp{\frac{L^{2/3}}{2} + O(L^{1/3}\log_2{L})} < 2^{L^{2/3}-1} = \abs{S}
\end{align*}
for large enough $L$. By the Pigeonhole Principle, there must be two distinct strings $\*x, \*y \in S$ such that $\phi(\*x), \phi(\*y)$ fall into the same sub-cube. In other words, we have
\begin{align*}
	\forall 0\le j< 2L^{1/3}, \quad \abs{a_j(\*x)-a_j(\*y)} \le 2^{-L^{1/3}/4}.
\end{align*} 
It follows that
\begin{align*}
	\sup_{z \in [1-8a,1]}\abs{g_{\*x}(z)-g_{\*y}(z)} &= \sup_{z \in [-1,1]}\abs{f_{\*x}(z)-f_{\*y}(z)} \\ 
	&\le \sup_{z \in [-1,1]}\sum_{j=0}^{L-k}\abs{a_j(\*x)-a_j(\*y)}\cdot\abs{T_j(z)} \\
	&\le \sum_{j=0}^{2L^{1/3}-1}2^{-L^{1/3}/4} + \sum_{j= 2L^{1/3}}^{L-k}2\cdot 2^{-L^{1/3}/4} \\
	&\le 2^{-L^{1/3}/5}.
\end{align*}
Let $a'=(\ln 2/75)L^{-2/3}<a$. Applying \cref{cor:ellipse-to-interval} to $g_{\*x}-g_{\*y}$ with $a=a'$ gives
\begin{align*}
	\sup_{z \in \partial \tE_{a',2}}\abs{g_{\*x}(z)-g_{\*y}(z)} &\le \exp\tp{5a'L/2} \cdot \sup_{z \in [1-8a,1]}\abs{g_{\*x}(z)-g_{\*y}(z)} \\
	&\le \exp\tp{5a'L/2} \cdot 2^{-L^{1/3}/10} \\
	&= 2^{L^{1/3}/30-L^{1/3}/10} = 2^{-L^{1/3}/15}.
\end{align*}
Let $\Gamma$ be the sub-arc of the circle $\set{p+qz\colon \abs{z}=1}$ which lies completely inside the ellipse $\tE_{a',2}$. Item (2) of \cref{prop:ellipse-bound} implies that the length of $\Gamma$ is at least $a'$. Therefore the Maximum Modulus Principle implies
\begin{align*}
	\sup_{\theta\colon \abs{\theta}\le \alpha L^{-2/3}}\abs{P_{\*e_k,\*x}(e^{i\theta})-P_{\*e_k,\*y}(e^{i\theta})} \le \sup_{z\in\Gamma}\abs{g_{\*x}(z)-g_{\*y}(z)} \le \sup_{z\in\tE_{a',2}}\abs{g_{\*x}(z)-g_{\*y}(z)} \le 2^{-L^{1/3}/15}.
\end{align*}
Here $\alpha=\ln{2}/150$. Now we have established the lemma for a fixed $k$-mer $w=\*e_k$. Since $\*x, \*y \in S$, \cref{lem:set-properties} says that for any other $k$-mer $w \in \set{0,1}^k$ either both $P_{w,\*x}(z)$ and $P_{w,\*y}(z)$ are zero polynomials or $w \in \set{0^k, \*e_1, \dots, \*e_k}$ and
\begin{align*}
    \sup_{\theta\colon \abs{\theta}\le \alpha L^{-2/3}}\abs{P_{w,\*x}(e^{i\theta})-P_{w,\*y}(e^{i\theta})} \le k\cdot \sup_{\theta\colon \abs{\theta}\le \alpha L^{-2/3}}\abs{P_{\*e_k,\*x}(e^{i\theta})-P_{\*e_k,\*y}(e^{i\theta})} \le 2^{-L^{1/3}/20}.
\end{align*}
Finally, we note that both $\*x$ and $\*y$ start with $\*s_0$, a run of 0s of length $L^{1/3}-1$.


\end{proof}

\begin{remark}
The key property of the strings in $S$ that allows the proof to go through is that any two 1's are separated by many 0's. If we define $S$ to be the set of $n$-bit strings where any two 1's are separated by at least $r\coloneqq L^{1/3}-1$ 0's, we can improve the size of $S$ to $2^{\Omega(L^{2/3}\log L)}$. This can be shown inductively, since the size of $S$ satisfies the recurrence relation $f(n)=f(n-1)+f(n-1-r)$. This can improve the bound in \cref{lem:technical-main} to $2^{-\Omega(L^{1/3}\sqrt{\log L})}$.
\end{remark}



==> openquestions.tex <==
\subsection{Open Questions} \enote{keep for ourselves?}

How do k-mer algorithms perform on average case models?

Is there a lower bound of $\Omega(n)T$ in the trace reconstruction using MLE?

